Probing Rotation of Core-collapse Supernova with Concurrent Analysis of Gravitational Waves and Neutrinos

The next time a core-collapse supernova (SN) explodes in our galaxy, vari- ous detectors will be ready and waiting to detect its emissions of gravitational waves (GWs) and neutrinos. Current numerical simulations have successfully introduced multi-dimensional effects to produce exploding SN models, but thus far the explosion mechanism is not well understood. In this paper, we focus on an investigation of progenitor core rotation via comparison of the start time of GW emission and that of the neutronization burst. The GW and neutrino de- tectors are assumed to be, respectively, the KAGRA detector and a co-located gadolinium-loaded water Cherenkov detector, either EGADS or GADZOOKS!. Our detection simulation studies show that for a nearby supernova (0.2 kpc) we can confirm the lack of core rotation close to 100% of the time, and the presence of core rotation about 90% of the time. Using this approach there is also po- tential to confirm rotation for considerably more distant Milky Way supernova explosions.

==> egads.tex <==
 EGADS detector is a Gadolinium doped water Cherenkov detector 
which is built for testing facilities and 
demonstrating the characterisics of GADZOOKS! project
and located in Kamioka Mine which is same mountain in SK and KAGRA.\\ 
 GADZOOKS! project is a project which adds 0.1$\%$ gadolinium (Gd) 
into the SuperKamiokande (SK) detector to detect the 
neutron from 
Inverse Beta Decay reaction($\bar{\nu_e} + p\to e^+ + n$), effectively.
Because of large cross section of Gd on the neutron capture,
and total energy of about 8MeV are emitted as multi gamma ray, 
we can identify by taking the coincidence between prompt positron 
signal and delayed gamma ray signal.\\
 EGADS detector consists of 200ton cylindrical tank, 
the height and radius are 7.0[m] and (WRITE HERE)[m], respectively.
Total 240 PMTs are placed inner wall, their coverage is 40$\%$.
This coverage is same vale as SuperKamiokande detector. 
 The 0.1$\%$ Gd corresponds to about 90$\%$ neutron tagging efficiency. 
Additional feature to identify inverse beta decay reaction is to 
collect pure electron scattering event, which means the 
better direction identification and Neutronization butst identification.
On 2010, the tank construction was finished, and commissional run was 
contined to check the water purification system, Gd doaping effect to 
materials. After installation of QBEE, which is same DAQ board as SK, 
the continuous observation will start. 


==> figs_revise.tex <==
\begin{figure}[ht]
 \centering
 \subfigure[$\nu_e$]{\includegraphics[width=0.8\textwidth]{./fig/neutrino.eps}}
 \subfigure[$\bar\nu_e$]{\includegraphics[width=0.8\textwidth]{./fig/antineutrino.eps}}
 \caption{Time evolution of luminosities of electron-type neutrinos
   ($\nu_e$; panel(a)) and antineutrinos ($\bar\nu_e$; panel
   (b)). Each line represents models with different initial rotation
   rates, i.e., no rotation($\Omega_0=0.0\pi$) (magenta), 
   $\Omega_0=0.2\pi$ rad s$^{-1}$
   (green), $\Omega_0=0.5\pi$ rad s$^{-1}$ (blue), and $\Omega_0=1.0\pi$
   rad s$^{-1}$ (red), respectively. 
   %!!! LINE COLORS SHOULD BE
   %CHANGED TO BE CONSISTENT WITH OTHER FIGURES!!! 
   %(done by Yokozawa 2014/05/28)
   Note that left and
   right sides in panel (a) have different scales.}
 \label{2-neutrino}
\end{figure}

\begin{figure}[ht]
 \centering
 \includegraphics[width=0.8\textwidth]{./fig/gw.eps}
 \caption{GW amplitude as a function of time for a core-collapse
   supernova occurring 10 kpc from the observer. Each line represents
   models with different initial rotation rate, i.e., no rotation
   ($\Omega_0=0.0\pi$)
   (magenta), $\Omega_0=0.2\pi$ rad s$^{-1}$ (green), $\Omega_0=0.5\pi$
   rad s$^{-1}$ (blue), and $\Omega_0=1.0\pi$ rad s$^{-1}$ (red),
   respectively. 
   %!!! LINE COLORS SHOULD BE CHANGED TO BE CONSISTENT
   %WITH OTHER FIGURES!!! 
   %(done by Yokozawa 2014/05/28)
   The small panel shows features around the bounce
   time. The fast rotation model exhibits a large amplitude GW at
   the bounce, while the slow rotation models have very
   small amplitudes. Since the later phase (i.e., a few tens of ms after
   the bounce) activity is dominated by convection motion, all
   models imply similar amplitude in the later phase.}
 \label{2-gw}
\end{figure}

\begin{figure}[ht]
 \centering
 \includegraphics[width=0.7\textwidth]{./fig/fig_kagra_noise.eps}
 \caption{KAGRA official sensitivity curve. These curves are estimated 
          from an incoherent sum of the fundamental noise sources. 
          The colors show each type of environmental noise and the black line shows 
          total noise. Blue lines are mirror related noise, brown shows seismic noise,
          green shows suspension thermal noise, and red shows quantum noise, respectively.}
 \label{fig:kagranoise}
\end{figure}


\begin{figure}[ht]
 \centering
 \includegraphics[width=0.7\textwidth]{./fig/fig_gw_oneshot.eps}
 \caption{One example of the time variation of obtained SNR for each model.
          Each color shows one progenitor core rotation model,
          0.0$\pi$(magenta), 0.2$\pi$(green), 0.5$\pi$(blue) 
          and 1.0$\pi$(red) rad s$^{-1}$, respectively.
          The supernova distance is set to 1.0 kpc and 
          on-direction for the KAGRA detector.
         }
 \label{fig/gw_oneshot}
\end{figure}

\begin{figure}[ht]
 \centering
 \includegraphics[width=0.7\textwidth]{./fig/fig_gw_sn_1kpc.eps}
 \caption{The max SNR distribution for each model.
          The supernova distance from Earth is fixed at 1kpc 
          and direction is randomly distributed.
          Each color shows one progenitor core rotation model,
          0.0$\pi$(magenta), 0.2$\pi$(green), 0.5$\pi$(blue) 
          and 1.0$\pi$(red) rad s$^{-1}$, respectively.
          The black line shows the detection threshold, which corresponds 
          to max SNR$>$8.}
 \label{fig/gw_sn_1kpc}
\end{figure} 


\begin{figure}[ht]
 \begin{minipage}[t]{0.49\textwidth}
  \includegraphics[width=\textwidth]{./fig/fig_gw_time_01kpc.eps}
  \caption{The {\cal T}$_{GW}$ extracted start time distribution 
          of GW emission for each explosion model. 
          The distance is fixed at 0.1kpc.
          Horizotal axis shows time from core bounce. 
          Each color shows one progenitor core rotation model,
          0.0$\pi$(magenta), 0.2$\pi$(green), 0.5$\pi$(blue) 
          and 1.0$\pi$(red) rad s$^{-1}$, respectively.}
  \label{fig/gw_time_01kpc}
 \end{minipage}
 \hspace{0.01\textwidth}
 \begin{minipage}[t]{0.49\textwidth}
  \includegraphics[width=\textwidth]{./fig/fig_gw_time_1kpc.eps}
  \caption{The {\cal T}$_{GW}$ distribution of GW emission for each explosion model. 
          The distance is fixed at 1.0 kpc.
          Horizotal axis shows time from core bounce. 
          Each color shows one progenitor core rotation model,
          0.0$\pi$(magenta), 0.2$\pi$(green), 0.5$\pi$(blue) 
          and 1.0$\pi$(red) rad s$^{-1}$, respectively.}
  \label{fig/gw_time_1kpc}
 \end{minipage}
\end{figure} 

\begin{figure}[ht]
 \centering
 \includegraphics[width=0.8\textwidth]{./fig/fig_gw_dfm_sample.eps}
 \caption{One example of the Dimmelmeier model, e20b-ls in the paper\citep{dfm}. 
          (Left) Time variation of gravitational wave amplitude h 
          as a function of time from core bounce for 10 kpc.
          (Right) Time variation of maximum density $\rho_{max}$.
          }
 \label{fig/gw_dfm_sample.eps}
\end{figure} 

\begin{figure}[ht]
 \begin{minipage}[t]{0.49\textwidth}
  \includegraphics[width=\textwidth]{./fig/fig_gw_dfm_eff.eps}
  \caption{The distance dependence of the detection efficiency 
          for Dimmelmeier 25 models.
          Black lines show each model and red points show 
          mean value and one sigma expansion
          of these models for each distance.
          }
  \label{fig/gw_dfm_eff.eps}
 \end{minipage}
 \hspace{0.01\textwidth}
 \begin{minipage}[t]{0.49\textwidth}
  \includegraphics[width=\textwidth]{./fig/fig_gw_dfm_time.eps}
  \caption{The distance dependence of the time 
          difference from core bounce time for Dimmelmeier 25 models.
          Black lines show for each model and red points show 
          mean value and one sigma expansion
          of these models for each distance. 
          }
  \label{fig/gw_dfm_time.eps}
 \end{minipage}
\end{figure} 

\begin{figure}[ht]
 \begin{minipage}[t]{0.49\textwidth}
  \includegraphics[width=\textwidth]{./fig/fig_nu_exp_evrate.eps}
  \caption{Expected number of interactions in EGADS. 
           Black component shows electron neutrino-electron elastic scattering, 
           blue component shows electron 
           anti-neturino-electron elastic scattering,
           and red component shows 10$\%$ of inverse beta decay interaction.
           Horizontal axis shows time and vertical 
           axis shows unit of event/1ms/10kpc.
          }
  \label{fig/exprate}
 \end{minipage}
 \hspace{0.01\textwidth}
 \begin{minipage}[t]{0.49\textwidth}
  \includegraphics[width=\textwidth]{./fig/fig_nu_exp_evrate_model.eps}
  \caption{Model dependence of expected number of summed interaction in EGADS. 
          Each color shows one progenitor core rotation model,
          0.0$\pi$(magenta), 0.2$\pi$(green), 0.5$\pi$(blue) 
          and 1.0$\pi$(red) rad s$^{-1}$, respectively.
          Horizontal axis shows time and 
          vertical axis is the sum of expected interactions in EGADS 
          in units of event/1ms/10kpc. }
  \label{fig/expratemodel}
 \end{minipage}
\end{figure}

\begin{figure}[ht]
 \begin{minipage}[t]{0.49\textwidth}
  \includegraphics[width=\textwidth]{./fig/fig_nu_oneshot.eps}
 \caption{One example of the fluctuation of observed number of neutrinos
          for the distance 0.1 kpc(red) and 0.5 kpc(blue). 
          The 1.0 $\pi$rad s$^{-1}$ model is used for this figure. 
          }
 \label{fig/nu_oneshot}
\end{minipage}
\hspace{0.01\textwidth}
\begin{minipage}[t]{0.49\textwidth}
 \includegraphics[width=\textwidth]{./fig/fig_nu_thres.eps}
 \caption{The number of maximum observed neutrinos used as threshold. 
          Colors show the progenitor core rotation models,  
          0.0$\pi$(magenta), 0.2$\pi$(green), 0.5$\pi$(blue) 
          and 1.0$\pi$(red) rad s$^{-1}$, respectively.
          Horizontal axis is number of observed events.
          }
 \label{fig/nu_thres}
 \end{minipage}
\end{figure}

\begin{figure}[ht]
 \centering
 \includegraphics[width=0.7\textwidth]{./fig/fig_nu_time_result.eps}
 \caption{The obtained {\cal T}$_{\nu}$ distribution in case of 0.1 kpc(red), 
          0.5 kpc(blue) and 1.0 kpc(green).}
 \label{fig/nu_time_result}
\end{figure}

\begin{figure}[ht]
 \begin{minipage}[t]{0.49\textwidth}
  \includegraphics[width=\textwidth]{./fig/fig_comp_time_01kpc_00.eps}
   \caption{Time comparison between {\cal T}$_{GW}$(red) 
            and {\cal T}$_{\nu}$(blue)
            distribution for 0.0$\pi$ rad s$^{-1}$ model. 
            The distance is fixed at 0.1 kpc. 
            Both GW and neutrino distributions are made
            after applying detection threshold. Horizontal axis shows time from 
            core bounce.}
  \label{fig/comp_time_01kpc_00}
 \end{minipage}
 \hspace{0.01\textwidth}
 \begin{minipage}[t]{0.49\textwidth}
  \includegraphics[width=\textwidth]{./fig/fig_comp_time_01kpc_10.eps}
  \caption{Time comparison between {\cal T}$_{GW}$(red) and 
           {\cal T}$_{\nu}$(blue)
           distribution for 1.0$\pi$ rad s$^{-1}$ model. 
           The distance is fixed at 0.1 kpc. 
           Both GW and neutrino distributions are made
           after applying detection threshold. Horizontal axis shows time from 
           core bounce.}
  \label{fig/comp_time_01kpc_10}
 \end{minipage}
\end{figure} 


\begin{figure}[ht]
 \centering
 \includegraphics[width=0.9\textwidth]{./fig/fig_comp_pr.eps}
 \caption{Model dependence of P$_r$ distribution, which is the probability of 
          core rotation.
          Horizotal axis shows distance. 
          Each color shows one progenitor core rotation model,
          0.0$\pi$(magenta), 0.2$\pi$(green), 0.5$\pi$(blue) 
          and 1.0$\pi$(red) rad s$^{-1}$, respectively.}
 \label{fig/comp_pr}
\end{figure} 



==> tables.tex <==

\begin{table}[h]
  \begin{center}
  \centering
  \caption{KAGRA detector coordinates.}
  \begin{tabular}{|c|c|}
    \hline
    parameter & value \\  \hline \hline
    latitude of KAGRA detector $\lambda$ & +36.41$^{\circ}$ \\ \hline
    longitude of KAGRA detector$L$ & +137.3$^{\circ}$ \\  \hline
    angle between East and bisector of the detector arms$\gamma$ & +75.0$^{\circ}$ \\ \hline
    angle between detector arms $\zeta$ & 90.0$^{\circ}$ \\ \hline
%%    \caption{aa}
  \end{tabular}
\label{tab/det_cor}     
  \end{center}
\end{table}

\begin{table}[h]
 \centering
 \caption{The distance dependence of GW, neutronization efficiency and $P_r$ value for 0.0$\pi$ rad/s model.}
  \begin{tabular}{|c| c| c| c| c|}
\hline
    Distance[kpc] & GW eff.[$\%$] & neutrino eff.[$\%$] & detection eff.[$\%$] & $P_r$[$\%$] \\ \hline \hline
0.1 & 71.9 & 100.0 & 71.9 & 0.0  \\  \hline
0.2 & 61.1 & 100.0 & 61.1 & 0.0  \\ \hline
0.3 & 52.5 & 100.0 & 52.5 & 0.4  \\ \hline
0.4 & 44.5 & 100.0 & 44.5 & 3.1  \\ \hline
0.5 & 39.6 & 100.0 & 39.6 & 8.6  \\ \hline
0.6 & 34.2 & 99.4  & 33.9 & 14.8 \\ \hline
0.7 & 29.9 & 93.0  & 27.6 & 21.3 \\ \hline
0.8 & 25.3 & 78.6  & 20.1 & 22.8 \\ \hline
0.9 & 22.7 & 58.6  & 13.6 & 28.0 \\ \hline
1.0 & 19.2 & 42.2  & 8.3  & 28.0 \\ \hline
%1.1 & 16.0 & 28.9  & 4.9  & 28.0 \\
%1.2 & 13.1 & 19.2  & 2.5  & 30.3 \\
%1.3 & 10.4 & 13.2  & 1.2  & 23.4 \\
%1.4 & 9.1  & 9.6   & 0.9  & 36.0 \\
1.5 & 7.3  & 6.3   & 0.4  & 35.6 \\ \hline
%1.6 & 6.1  & 4.5   & 0.3  & 28.0 \\
%1.7 & 4.0  & 3.7   & 0.1  & 33.3 \\
%1.8 & 3.5  & 2.2   & 0.1  & 0.0  \\
%1.9 & 2.8  & 1.9   & 0.1  & 28.6 \\
2.0 & 1.9  & 1.3   & $<$0.1 & 25.0 \\ \hline
  \end{tabular}
  \label{tab/suwa00}
\end{table}


\begin{table}[h]
 \centering
 \caption{The distance dependence of GW, neutronization efficiency and $P_r$ value for 0.2$\pi$ rad/s model.}
  \begin{tabular}{|c| c| c| c| c|}
\hline
    Distance[kpc] & GW eff.[$\%$] & neutrino eff.[$\%$] & detection eff.[$\%$] & P$_r$[$\%$] \\ \hline \hline
0.1 & 71.9 & 100.0 & 71.9 & 0.0  \\ \hline
0.2 & 61.0 & 100.0 & 60.9 & 1.3  \\ \hline
0.3 & 52.1 & 100.0 & 52.1 & 5.3  \\ \hline
0.4 & 44.9 & 100.0 & 44.9 & 13.6 \\ \hline
0.5 & 39.1 & 100.0 & 39.1 & 22.4 \\ \hline
0.6 & 34.2 & 98.9  & 33.7 & 29.9 \\ \hline
0.7 & 29.8 & 89.7  & 26.7 & 38.1 \\ \hline
0.8 & 24.2 & 70.6  & 17.1 & 42.6 \\ \hline
0.9 & 21.5 & 51.8  & 11.3 & 41.8 \\ \hline
1.0 & 18.8 & 35.3  & 6.7  & 40.3 \\ \hline
%1.1 & 16.1 & 23.4  & 3.8  & 45.7 \\
%1.2 & 12.9 & 16.2  & 2.2  & 44.0 \\
%1.3 & 10.2 & 11.1  & 1.1  & 43.9 \\
%1.4 & 8.2  & 7.6   & 0.6  & 37.5 \\
1.5 & 6.5  & 4.8   & 0.2  & 27.3 \\ \hline
%1.6 & 5.1  & 3.6   & 0.3  & 29.0 \\
%1.7 & 4.4  & 2.6   & 0.1  & 35.7 \\
%1.8 & 3.2  & 2.0   & $<$0.1 & 33.3 \\
%1.9 & 2.7  & 1.1   & $<$0.1 & 50.0 \\
2.0 & 1.9  & 0.9   & $<$0.1 & 0.0  \\ \hline
  \end{tabular}
  \label{tab/suwa02}
\end{table}


\begin{table}[h]
 \centering
 \caption{The distance dependence of GW, neutronization efficiency and $P_r$ value for 0.5$\pi$ rad/s model.}
  \begin{tabular}{|c |c |c |c |c|}
 \hline
    Distance[kpc] & GW eff.[$\%$] & neutrino eff.[$\%$] & detection eff.[$\%$] & P$_r$[$\%$] \\ \hline \hline
0.1 & 84.9 & 100.0 & 84.9 & 0.2  \\ \hline
0.2 & 77.7 & 100.0 & 77.7 & 1.8  \\ \hline
0.3 & 73.7 & 100.0 & 73.7 & 8.5  \\ \hline
0.4 & 69.6 & 100.0 & 69.6 & 17.1 \\ \hline
0.5 & 65.1 & 100.0 & 65.1 & 26.1 \\ \hline
0.6 & 62.8 & 99.0  & 62.2 & 33.9 \\ \hline
0.7 & 60.3 & 91.4  & 55.5 & 40.0 \\ \hline
0.8 & 56.6 & 75.0  & 42.8 & 44.0 \\ \hline
0.9 & 54.1 & 55.1  & 29.7 & 48.0 \\ \hline
1.0 & 52.5 & 38.8  & 20.3 & 47.3 \\ \hline
%1.1 & 50.7 & 26.5  & 13.1 & 46.6 \\
%1.2 & 46.8 & 18.0  & 8.7  & 46.3 \\
%1.3 & 46.0 & 12.3  & 5.6  & 44.6 \\
%1.4 & 43.3 & 8.6   & 3.5  & 45.6 \\
1.5 & 43.0 & 6.1   & 2.6  & 45.6 \\ \hline
%1.6 & 40.9 & 4.1   & 1.7  & 46.4 \\
%1.7 & 37.9 & 3.1   & 1.4  & 42.6 \\
%1.8 & 38.0 & 2.2   & 0.8  & 35.1 \\
%1.9 & 36.0 & 1.9   & 0.6  & 33.3 \\
2.0 & 35.1 & 1.1   & 0.3  & 35.5 \\ \hline
  \end{tabular}
  \label{tab/suwa05}
\end{table}

\begin{table}[h]
 \centering
 \caption{The distance dependence of GW, neutronization efficiency and $P_r$ value for 1.0$\pi$ rad/s model.}
  \begin{tabular}{|c |c |c |c |c|}
 \hline
    Distance[kpc] & GW eff.[$\%$] & neutrino eff.[$\%$] & detection eff.[$\%$] & P$_r$[$\%$] \\ \hline \hline
0.1 & 87.2 & 100.0 & 87.2 & 95.8 \\ \hline
0.2 & 82.0 & 100.0 & 82.0 & 92.6 \\ \hline
0.3 & 78.3 & 100.0 & 78.3 & 90.1 \\ \hline
0.4 & 74.6 & 100.0 & 74.6 & 88.6 \\ \hline
0.5 & 72.3 & 100.0 & 72.3 & 86.8 \\ \hline
0.6 & 69.6 & 98.1  & 68.1 & 87.3 \\ \hline
0.7 & 67.4 & 87.0  & 58.6 & 87.0 \\ \hline
0.8 & 65.1 & 68.0  & 44.5 & 85.7 \\ \hline
0.9 & 63.0 & 49.1  & 30.7 & 85.9 \\ \hline
1.0 & 61.0 & 34.1  & 20.9 & 85.8 \\ \hline
%1.1 & 59.3 & 23.3  & 13.9 & 82.6 \\
%1.2 & 57.4 & 15.3  & 9.0  & 83.4 \\
%1.3 & 55.3 & 10.9  & 6.1  & 83.7 \\
%1.4 & 54.2 & 7.6   & 4.2  & 80.0 \\
1.5 & 52.8 & 5.7   & 3.2  & 83.8 \\ \hline
%1.6 & 51.1 & 3.8   & 1.8  & 72.9 \\
%1.7 & 49.9 & 2.8   & 1.3  & 75.9 \\
%1.8 & 48.0 & 2.1   & 1.0  & 73.8 \\
%1.9 & 47.1 & 1.7   & 0.7  & 75.3 \\
2.0 & 45.8 & 1.3   & 0.7  & 69.6 \\ \hline
  \end{tabular}
  \label{tab/suwa10}
\end{table}

